NEUZZ: Efficient Fuzzing with Neural Program Smoothing

Fuzzing has become the de facto standard technique for finding software vulnerabilities. However, even state-of-the-art fuzzers are not very efficient at finding hard-to-trigger software bugs. Most popular fuzzers use evolutionary guidance to generate inputs that can trigger different bugs. Such evolutionary algorithms, while fast and simple to implement, often get stuck in fruitless sequences of random mutations. Gradient-guided optimization presents a promising alternative to evolutionary guidance. Gradient-guided techniques have been shown to significantly outperform evolutionary algorithms at solving high-dimensional structured optimization problems in domains like machine learning by efficiently utilizing gradients or higher-order derivatives of the underlying function. However, gradient-guided approaches are not directly applicable to fuzzing as real-world program behaviors contain many discontinuities, plateaus, and ridges where the gradient-based methods often get stuck. We observe that this problem can be addressed by creating a smooth surrogate function approximating the discrete branching behavior of target program. In this paper, we propose a novel program smoothing technique using surrogate neural network models that can incrementally learn smooth approximations of a complex, real-world program's branching behaviors. We further demonstrate that such neural network models can be used together with gradient-guided input generation schemes to significantly improve the fuzzing efficiency. Our extensive evaluations demonstrate that NEUZZ significantly outperforms 10 state-of-the-art graybox fuzzers on 10 real-world programs both at finding new bugs and achieving higher edge coverage. NEUZZ found 31 unknown bugs that other fuzzers failed to find in 10 real world programs and achieved 3X more edge coverage than all of the tested graybox fuzzers for 24 hours running.

==> RQ_tab.tex <==
% \begin{table*}[t]
% %\setlength{\tabcolsep}{6pt}
% \renewcommand{\arraystretch}{1.1}
%   \caption{Code coverage of 1M mutations generated by \sys and AFL}
%   \label{tab:1m}
% \parbox{.46\linewidth}{
% \centering
% \subfloat[New code coverage while running AFL for 1 hour to generate the training data]{

% \begin{tabular}{l|cc|cc}
%     \hline
%   \multirow{2}{*}{Programs}  & \multicolumn{2}{c|}{Line coverage} & \multicolumn{2}{c}{Edge coverage}\\\cline{2-5}
%     & \sys  & AFL & \sys & AFL\\ 
%     \hline
%     readelf -a & 1,412 & 183 & 2,378& 213  \\
%     nm -C & 40 & 0 & 120 & 56\\
%     objdump -D & 82 & 0 & 140 & 1\\
%     size & 67 & 0 &180 & 3\\
%     strip & 75 & 0 & 407 & 1\\
%     libjpeg & 160 & 19 & 142 & 28 \\
%     libxml & 204 & 5 & 273 & 19 \\
%     mupdf &  28 & 0 & 121 & 32 \\
%     zlib & 138 & 5 & 174  &53 \\
%     harfbuzz & 284 & 0 & 1,014 & 27 \\
%   \hline
% \end{tabular}
% \label{tab:1h_1m}
% }
% }
% \hspace{.2cm}
% \parbox{.46\linewidth}{
% \centering
% \subfloat[New code coverage while running AFL for 6 hours to generate the training data]{
%  \begin{tabular}{l|cc|cc}
%     \hline
%  \multirow{2}{*}{Programs}  & \multicolumn{2}{c|}{Line coverage} & \multicolumn{2}{c}{Edge coverage}\\\cline{2-5}
%     & \sys  & AFL & \sys & AFL\\ 
%     \hline
%     readelf -a &1,569 &0 & 2,451& 4 \\
%     nm -C & 145 & 0 & 174 & 0\\
%     objdump -D & 58 & 2 &  187&8 \\
%     size & 33 & 0 &177 & 0\\
%     strip & 71 & 0 &  311& 21\\
%     libjpeg &  294 & 0 & 126 & 0 \\
%     libxml & 87 & 0 & 133 & 0\\
%     mupdf & 15 & 0 & 63 & 0\\
%     zlib & 97 & 0 & 161 & 0\\
%     harfbuzz & 52  & 0 & 322 & 0\\
%   \hline
% \end{tabular}
% \label{tab:6h_1m}
% }
% }
% \end{table*}


\begin{table}[!htpb]
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{1.1}
\centering
\caption{\textbf{\small Code coverage of 1M mutations generated by \sys and AFL}}
\label{tab:1m}
\begin{tabular}{lrr|rr|rr|rr}
   \toprule
   & \multicolumn{4}{c|}{1 hour corpus} & \multicolumn{4}{c}{6 hour corpus} \\ \cline{2-9}
   \multirow{2}{*}{Programs}  & \multicolumn{2}{c|}{Line coverage} & \multicolumn{2}{c|}{Edge coverage} & \multicolumn{2}{c|}{Line coverage} & \multicolumn{2}{c}{Edge coverage}\\ \cline{2-9}
    & \sys  & AFL & \sys & AFL & \sys  & AFL & \sys & AFL \\ 
    \hline
    readelf -a & 1,412 & 183 & 2,378& 213  &1,569 &0 & 2,451& 4  \\
    nm -C & 40 & 0 & 120 & 56 & 145 & 0 & 174 & 0\\
    objdump -D & 82 & 0 & 140 & 1 & 58 & 2 &  187&8\\
    size & 67 & 0 &180 & 3& 33 & 0 &177 & 0\\
    strip & 75 & 0 & 407 & 1& 71 & 0 &  311& 21\\
    libjpeg & 160 & 19 & 142 & 28 &  294 & 0 & 126 & 0\\
    libxml & 204 & 5 & 273 & 19 & 87 & 0 & 133 & 0\\
    mupdf &  28 & 0 & 121 & 32& 15 & 0 & 63 & 0 \\
    zlib & 138 & 5 & 174  &53& 97 & 0 & 161 & 0 \\
    harfbuzz & 284 & 0 & 1,014 & 27 & 52  & 0 & 322 & 0\\
  \bottomrule
\end{tabular}
\label{tab:1h_1m}
%}
%}
% \hspace{.2cm}
% \parbox{.46\linewidth}{
% \centering
% \subfloat[New code coverage while running AFL for 6 hours to generate the training data]{
%  \begin{tabular}{l|cc|cc}
%  \toprule
%  \multirow{2}{*}{Programs}  & \multicolumn{2}{c|}{Line coverage} & \multicolumn{2}{c}{Edge coverage}\\\cline{2-5}
%     & \sys  & AFL & \sys & AFL\\ 
%     \hline
%     readelf -a &1,569 &0 & 2,451& 4 \\
%     nm -C & 145 & 0 & 174 & 0\\
%     objdump -D & 58 & 2 &  187&8 \\
%     size & 33 & 0 &177 & 0\\
%     strip & 71 & 0 &  311& 21\\
%     libjpeg &  294 & 0 & 126 & 0 \\
%     libxml & 87 & 0 & 133 & 0\\
%     mupdf & 15 & 0 & 63 & 0\\
%     zlib & 97 & 0 & 161 & 0\\
%     harfbuzz & 52  & 0 & 322 & 0\\
%   \bottomrule
% \end{tabular}
%\label{tab:6h_1m}
%}
%}
% \tableshrink
\end{table}

==> cgc.tex <==
The DARPA CGC data set~\cite{cgc_corpus} consists of vulnerable programs used in the Cyber Grand Challenge. These programs are implemented as network services which performing various tasks, aimed to mirror real world applications with known vulnerabilities. Every bug in the programs is guarded by a number of sanity checks on the input and is also provided with a set of inputs as proof of vulnerability.

We evaluate \sys and \afl on three cgc binary \texttt{KPRCA00001}, \texttt{CROMU_00027}, and \dng{find the third case} for three hours. For \sys, we split one hour time budget to collect training data by \aflintel and the remaining two hour to generate mutations. Since the bugs in all 3 programs are guarded by a number of sanity checking, we provide the initial seed which can reach the sanity checking for both fuzzers. The results show that \sys can find bugs in all 3 programs within 10 minutes by efficiently solving the magic number condition through gradient-guided local exhaustive searching. While \afl fails to find any bugs in all 3 programs because the complex magic number condition are hard to break by random evolutionary fuzzing with any pre-computed fuzzing dictionary.

 \lstset{style=braystyle}
 \label{cgc_code}
 \begin{lstlisting}[caption={\textbf{\small The cgc_ReceiveCommand function in CROMU_00027}}, captionpos=b, label={lst:run_ex}, float=h]
 int cgc_ReceiveCommand(CommandStruct *command, int *more_command) {
 ...
 if (cgc_strncmp(&buffer[1], "VISUALIZE", cgc_strlen("VISUALIZE")) == 0) {
    command->command = VISUALIZE;
    //vulnerable code
...
\end{lstlisting}
We analyze a example program in detail. \texttt{CROMU_00027} is a ASCII content server which takes query from client and serves all outputs as ASCII code. The bug a null-pointer deference in the serve content function is triggered when user try to visualize a invalid content with NULL pointer. The magic string comparison is extremely hard for \afl to break, so it failed to detect this bug within 3 hour time budget. \sys can leverage the gradient-guided information to locate the critical bytes in the program which determine the magic comparison, then perform a efficient local exhaustive searching to break it. 

==> disclosure.tex <==
\vspace*{20px}
\noindent\fbox{\begin{minipage}{24em}
{\bf Vulnerability Disclosure}: We are currently in the process of notifying the developers of the affected programs. Please treat the bugs as confidential and do not disclose any information about them.
\end{minipage}}

==> overview_bckup.tex <==
\section{Neural Fuzzing Overview}
\label{sec:overview}

In this section, we begin with introducing the challenges of existing fuzzing techniques that motivate us to use learning enabled fuzzing. 
We then discuss the challenges of modeling fuzzing as a learning problem. We further present different design choices of neural network (NN) architectures and their pros and challenges in modeling program logic.
Finally, we describe the workflow of our system, \sys, along with a running example.


\subsection{Fuzzing as a Learning Problem}

While traditional fuzzing techniques have shown great success in finding security vulnerabilities, nearly all of them needs to consider the tradeoff between the efficiency (\ie scalability to large programs) and effectiveness (\ie generating high-quality inputs covering diverse code branches).
For example, a state-of-the-art security fuzzer, \afl~\cite{zalewski2007american}, employs genetic algorithm to efficiently mutate test seeds. 
Despite proved to be efficient in generating test inputs, it often gets stuck and fails to find new branches after several hours of running (see Section~\ref{sec:eval} for details).
Other more principled mutation-guiding strategies such as symbolic execution~\cite{stephens2016driller} leverage more fine-grained program information to direct the input generation towards uncovered branches. However, the overhead of these whitebox techniques can become prohibitive when dealing with the combinatorial paths of the increasingly complex program.

% The reason is that AFL apply a uniform random mutation procedure during whole fuzzing process and never learn from past millions of execution experience. For example, during the beginning of fuzzing, AFL would generate a large number of invalid mutations by either flipping the magic number section or other constant values in the file header; after several hours of fuzzing, it would still generate a large number of invalid mutations from any parent seeds. 

In this paper, we explore the potential of learning-based fuzzing, which seeks for a good balancing between the effectiveness in generating high-quality fuzzing inputs (\ie precisely guiding the mutation) and the efficiency (\ie in terms of the number of inputs generated within a limited time frame)
~\bray{What is the intuition behind using learning based approach?}.
~\kx{I try to explain the intuition in the following with two bold bullets.}

In particular, we train NN to (approximately) represent the program logic. Then based on the trained NN, we model the mutation of input to look for new code coverage as an optimization problem, and leverage the gradient of the trained network (a continuous differentiable function) to efficiently compute the critical locations of the input to mutate.
There are two important intuitions of doing this and we describe in detail in the following.

\noindent\textbf{Differentiable program representation.}
The first advantage of differentiable representation of the program enables leveraging gradient to maximize certain output of the program with respect to the input.
Our rationale of using NN to emulate the program logic is based on the universal approximation theorem~\cite{hornik1991approximation}.
Essentially, a multi-layer neural network is capable to approximate arbitrary functions given enough training data.
In addition, gradient computation within the NN (\ie to support back propagation) is fairly efficient powered by GPU.
Therefore, if a discrete program based on control sequences (essentially a function) can be represented by a continuous differentiable NN, we can transform the branch searching problem (\ie a combinatorial constraints solving) into a numerical optimization problem.

Indeed, the approximation of using NN to represent program logic sacrifices accuracy to some extent (\ie does not exactly map the NN logic to the program logic).
Our hope is this style of inaccurate modeling can still provides more reasonable guidance in mutation than heuristics (\eg evolutionary approach), while also incurs less overhead as compared to the fine-grained program analysis (\eg symbolic execution).
In the next section, we describe our modeling of NN in approximating program logic, and in Section~\ref{sec:methodology}, we give the detail how to the compute the gradient to efficiently locate the critical input parts to mutate.

\noindent\textbf{Rich training sources.} 
While differentiable program representation enables efficient computation of critical mutation location, the core prerequisite is that the NN representation should \textit{approximate the real discrete program as close as possible}.
Otherwise, the computed gradient will not effectively emulate the criticalness of the input to guide the mutation.
Fortunately, the rich source of training samples are available that can help the NN to be trained to mimic the real program
The training samples can be drawn cheaply by using random fuzzing.
Specifically, after defining the input-output format of the NN, the training data can be easily collected through running random testing for a while.
We give the details of the format of the input-output we used in this paper in the following.

\subsection{Modeling Challenges}
Despite the advantages of learning-based fuzzing described above, applying machine learning to guide fuzzing is fundamentally a hard problem.
This requires nontrivial effort in carefully encoding the fuzzing problem and engineering the features to closely model the fuzzing tasks (\ie improving branch coverage, path coverage, etc.).
For example, a naive encoding of fuzzing is treating the input as raw bytes and the output as a single value denoting the coverage percentage.
Then the optimization problem becomes finding inputs that can maximize the output.
However, as the code coverage is a stateful cumulative measurement, how to compute a combination of inputs to have the cumulatively highest coverage is problematic in this encoding.

In the following, we describe potential input-output modeling choices where part of them are also employed in the literature and also our feature engineering strategy.

\noindent\textbf{Input representation.}
Engineering the features to represent the input to the program can be done in different granularity.
The finest-grained method is to treat every input as raw bytes and each byte encodes one feature with possible values between 0 and 255.
A more coarse-grained but smarter features leverage the domain knowledge of the input structure, such as grammar-based abstract syntax tree~\cite{wang2017skyfire} or the objects of specific type of input (\eg PDF)~\cite{godefroid2017learn}.

In this work, we seek to fully exploit the NN's extraordinary capability in extracting hidden patterns from raw level input (\eg bytes, pixels)~\cite{yosinskiunderstanding}. Therefore, we choose to take the raw byte as the input features.

\noindent\textbf{Output representation.}
Recall our task is to learn an NN to approximate the program, and then query the learned NN to get the mutation guidance to achieve higher coverage.
Therefore, we model the output of the NN to directly represent the coverage information
the output of the NN can be the covered lines given input, where each output neuron in the final layer denotes one line and the output value of the neuron denotes whether the line is covered or not (\ie 1 denotes covered while 0 denotes not covered). 
Then the task is to leverage this trained NN to find inputs that can cover lines that were not covered before.
Considering the large number of potential lines of the real-world programs, we resort to encode each branch as one of the neuron
As such, the NN is a multi-input and multi-output function mapping the raw bytes of the program input to the corresponding branch coverage of the program.

\noindent\textbf{NN models.}

\subsection{Design Choices of Neural Architecture}
What kind of modeling options
Scalability, hard to train, etc.
Picture 1, picture 2, illustration

1. Efficiency (training time), 
	In terms of modeling
    In terms of computing gradient
    Random vs AFL vs RL vs RNN vs Ours
    Scalability (timeout vs time)
2. Effectiveness (same time/same \# generated input code)
    gradient also helps (better way of genetic)
    RQ: gradient based is a new way of guiding fuzzing

\noindent\textbf{Feedforward CNN.}

\noindent\textbf{Sequence-to-sequence (seq2seq) RNN.}

\noindent\textbf{Reinforcement learning.}

\subsection{\sys Workflow}



==> rq11.tex <==
% \RQA{3}{Does \sys find more crashes and bugs than AFL?} 
\medskip
\noindent
\textbf{(i) Detecting real-world bugs.}
We compare the total number of bugs and crashes found by \sys and other fuzzers on 1 hour running time given 6 hours of seed corpus. 
There are four different types of bugs found by \sys and other fuzzers: out-of-memory, memory leak, crash, and integer overflow. To detect memory bugs that would not necessarily lead to a crash, we compile program binaries with address sanitizer~\cite{asan}. We measure the unique memory bugs found by comparing the stack traces reported by the address sanitizer. For crashes that do not cause a bug report to be generated by the address sanitizer, we examine the execution trace. The integer overflow bugs are found by manually analyzing the inputs that trigger an infinite loop. 
We further verify integer overflow bugs using the undefined behavior sanitize~\cite{usan}.
The results are summarized in Table ~\ref{tab:bug_summary}. 

\input{tables/realworld_bug.tex}

 \sys finds all the $4$ types of bugs across $6$ programs. \aflfast and \lafintel find $3$ types of bugs\textemdash they do not find any interger overflow bugs.  
 %(memory leak, out-of-memory and crash) on $5$ programs. 
 The other fuzzers only find $2$ types of bugs (\ie, memory leak and crash). In total, \sys finds $2\times$ more bugs than the second best fuzzer. Moreover, the integer-overflow vulnerability  in \texttt{strip}, which is only found by \sys, is confirmed and getting fixed by the developers. 

% The exclusive bugs found by \sys is a integer-overflow bug in \texttt{strip} and out-of-memory bug in \texttt{libjpeg}. The crashes in program \texttt{readelf} are found by \aflfast, \lafintel and \sys. Moreover, \sys finds $6$ unique crashes in program \texttt{readelf}, while \aflfast and \lafintel can only find $1$ crash in \texttt{readelf}. We will discuss them in detail in Section~\ref{sec:case_study}. As for memory reported by the address sanitizer, \sys finds memory leaks in $3$ programs (\texttt{readelf}, \texttt{objdump} and \texttt{strip}) and out-of-memory bugs in $5$ programs (\texttt{objdump}, \texttt{size}, \texttt{strip}, \texttt{nm} and \texttt{libjpeg}), while other fuzzers can also memory leaks in $3$ programs (\texttt{readelf}, \texttt{objdump} and \texttt{strip}) and out-of-memory bugs in $4$ programs (\texttt{objdump}, \texttt{size}, \texttt{strip}, \texttt{nm}). \sys is able to find all the memory bugs that other fuzzers finds along with additional memory leaks in $3$ programs and out-of-memory bugs in $2$ programs. We think it is because \sys implements the effective local exhaustive searching on the critical bytes of program inputs which are more likely to try the extreme value of variables used in the program and trigger the memory bugs. In summary, \afl shows great ability to find the real-world bugs, \aflfast and \lafintel achieve the a little bit lower bug number than \afl but find a additional crash which \afl fails to find. \vuzzer performs worst because \vuzzer can only generate a small number of mutations during 1 hour running time. Meanwhile, \vuzzer's mutation strategy is to generate promising inputs by copy the magic constants into the corresponding input locations, which is not effective to trigger any out-of-memory bugs which occurs frequently in most of binutils programs. \kleefl finds the second-least bug number. We think it is because \kleefl takes additional seeds generated by klee which may distract most of fuzzing energy to those rare branches and didn't fully explore the buggy common branches. In total, \sys finds the maximum number of bugs among all $6$ fuzzers.

\RS{1}{\sys found 30 previously unknown bugs in 6 different programs that other fuzzers could not find.}

%\begin{table}[!t]
%\setlength{\tabcolsep}{5pt}
%\centering
%\renewcommand{\arraystretch}{1.1}
%\caption{\textbf{\small Number of bugs found by \afl and \sys. We use $x/y$ to denote the number of bugs found by \sys and \afl, respectively, when they differ}}
%\label{tab:bug_summary}
%\begin{tabular}{l|cccc|cc}
%\hline
%Programs & \begin{tabular}[c]{@{}c@{}}Mem\\ leak\end{tabular} & \begin{tabular}[c]{@{}c@{}}Out\\ mem\end{tabular} & \begin{tabular}[c]{@{}c@{}}Interger\\ overflow\end{tabular} & Crash & \begin{tabular}[c]{@{}c@{}}\sys\\ Total\end{tabular} & \begin{tabular}[c]{@{}c@{}}\afl\\ Total\end{tabular} \\ \hline
%readelf & 10/4 & 0 & 0 & 6/0 & 16  & 4  \\
%nm & 0 & 8/8 & 0 & 0  & 8 & 8  \\
%objdump & 2/0 & 6/6 &0  & 0&  8 & 6   \\
%size & 0 & 5/3 & 0 & 0 &  5 & 3  \\
%strip & 5/1 & 14/6 & 7/0 & 0 &  26 & 7 \\
%libjpeg & 0 & 1/0 & 0 & 0 &  1 & 0  \\
%\bottomrule
%\end{tabular}
%\tableshrink
%\end{table}





==> rq12.tex <==
\medskip
\noindent
\textbf{(ii)~Detecting injected bugs in LAVA-M dataset.} 
LAVA dataset is created to evaluate the efficacy of fuzzers by providing a set of real-world programs injected with a large number of realistic bugs~\cite{lava}. LAVA-M is a subset of LAVA datasets, consisting of $4$ GNU coreutil programs {\tt base64}, {\tt md5sum}, {\tt uniq}, and {\tt who} injected with $44$, $57$, $28$, $2136$ bugs respectively. All the bugs are guarded by a four-bytes magic number comparison. If the condition is satisfied, then the bug number will be printed out. We compare \sys's performance to find these bugs \wrt other state-of-art fuzzers, as shown in~\Cref{tab:lava}. 
Following the conventional practices~\cite{angora,lava}, we use $5$ hours time budget for all the fuzzers. 
%, including a coverage-guided fuzzer (FUZZER), a symbolic execution tool (SES)~\cite{lava}, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix}, Angora~\cite{angora}, and T-fuzz~\cite{tfuzz}.
%We compare \sys with all these fuzzers, and the results are summarized in~\Cref{tab:lava}.

Triggering a magic number condition is a hard task for a coverage-guided fuzzer because the fuzzer has to generate the exact combination of four continuous bytes out of $256^4$ possible cases.  To solve this program, we use \lafintel to transform a magic byte comparison into four nested byte-comparisons. % and thus, reducing the search space from $256^4$ to $256$. 
We run \lafintel for four hours to generate the training data, then train a neural program whose gradients identify the possible critical bytes triggering the first byte-comparison of a magic-byte condition. After that, we perform a locally exhaustive search on each byte adjacent to the first critical bytes to break the second byte-comparison in $256$ tries, and then another $256$ tries to break the third byte-comparison, then the last $256$ tries to break the fourth byte-comparison.
Therefore, we need 1-time gradient computation and $26368$ tries to trigger each bug.
For program {\tt md5sum}, following the latest suggestion of the LAVA-M's authors, we further  reduce the seed into a single line, which greatly boost the fuzzing performance. 
%We also observed promising results by \lafintel itself when collecting the training data. So we re-split 4 hours time budget to \lafintel to collect the training data and leave 1 hour to perform efficient searching guided by neural program.  

%LAVA-M dataset has been evaluated by multiple state-of-the-art fuzzers with $5$ hours time budget, including a coverage-guided fuzzer (FUZZER), a symbolic execution tool (SES)~\cite{lava}, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix}, Angora~\cite{angora}, and T-fuzz~\cite{tfuzz}.
%As shown in~\ref{tab:lava},
%We compare \sys with all these fuzzers, and the results are summarized in~\Cref{tab:lava}. %\lafintel performs remarkably well during the 5 hours fuzzing process, as shown in~\Cref{tab:lava}. 
% \sys finds all the bugs in programs {\tt base64}, {\tt md5sum}, and {\tt uniq}, and second highest bug number in program who.  Note that LAVA-M authors left some bugs unlisted in all $4$ programs, so the total number of bugs found by \sys can be higher than the number of listed bugs. 

% LAVA-M dataset has been evaluated by multiple state-of-the-art fuzzers with $5$ hours time budget, including a coverage-guided fuzzer (FUZZER), a symbolic execution tool (SES)~\cite{lava}, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix}, Angora~\cite{angora}, and T-fuzz~\cite{tfuzz}.
% We compare \sys with all these fuzzers and the result are summarized in table~\ref{tab:lava}. We also observed great results by AFL-lafintel when collecting training data, so we listed the 5 hours fuzzing result of AFL-lafintel on the table. \sys finds all the bugs in programs base64, md5sum and uniq, and second highest bug number in program who.  Note that LAVA-M authors left some bugs unlisted in all $4$ programs, so the total number of bugs found by \sys can be higher than the number of listed bugs. We explain the reason for \sys's promising results as follows. 

As shown in~\ref{tab:lava},
\sys finds all the bugs in programs {\tt base64}, {\tt md5sum}, and {\tt uniq}, and the  highest number of bugs for program {\tt who}.  
Note that LAVA-M authors left some bugs unlisted in all $4$ programs, so the total number of bugs found by \sys can be higher than the number of listed bugs, as shown in the result.
There are several reasons behind \sys's success. First, our design choice breaks the search space in multiple manageable steps: sys trains the underlying NN on the \lafintel generated data, uses the computed gradient to reach the first critical byte, and performs a local search around the found critical region. 

%First, all the bugs in LAVA-M datasets, guarded by a four-byte magic number condition, can be triggered by four consecutive bytes in the program input. \sys uses AFL-lafintel to transform the four-byte magic number comparison into four nested byte-comparisons. AFL-lafintel can easily trigger the first byte-comparison easily by randomly fuzzing, but it cannot locate the critical byte which determines the first byte-comparison. Given the program inputs generated by AFL-lafintel, \sys can learn a neural program which help identify the possible critical bytes in the program inputs leading to first byte-comparisons. Then it just need another $256*3$ tries to perform a local exhaustive search to break the complex magic number comparisons, which greatly reduces the searching space. However, the transformation of magic number comparison by \lafintel would cause a potential edge explosion issue for programs with a large number of compare instructions. The large number of edges emitted by \lafintel would cause frequent edge conflict in the AFL edge map. This explains why \lafintel cannot find any bugs in program {\tt who}. %, and edge explosion also affects \sys performance on program who. 

\input{tables/lava.tex} 

%Second, most of fuzzers (except) fail to find most of bugs in program md5sum because the improper seed provided by LAVA-M would cause the program to run slowly. We followed the latest suggestion on the authors of LAVA-M's blog, reduce the seed of md5sum into a single line, which greatly boost the fuzzing performance. 

Secondly, compared with Steelix and \vuzzer, which leverage magic number hard-coded in the binary to construct a program inputs, \sys's exhaustive searching strategy does not rely on any hard-coded magic number. 
Thus, it can find all the bugs in program {\tt md5sum},  which requires some computations of input bytes to do the magic number checking. Compared with Angora, the current state-of-the-art fuzzer for LAVA-M dataset, \sys finds $3$ more bugs in program {\tt md5sum}, because \sys does not need to solve the complex magic number condition at one time.
As long as it can trigger the first byte-comparisons of a magic number condition, it can trigger the bug quickly. While Angora have to solve every complex magic number conditions and it is hard to hit all of them given fixed time budget. 


%Angora finds $1541$ in program who, while \sys only find $211$ bugs because AFL-lafintel transformation generates too many additional edges which cause a sever edge conflict issue. We try to expand the edge map size to mitigate this issue, but find that AFL-lafintel cannot fully explore all the first byte-comparisons of all $2136$ magic number comparisons within limited time budget, which limit the accuracy of neural programs learnt from pro rams inputs generated by AFL-lafintel. 
                  
%\input{RQ_tab}
\input{RQ_fig}

==> rq1_old.tex <==
%\rqsection{Is \sys more efficient to explore code coverage than AFL?}
\RQA{1}{How does \sys perform on LAVA data sets?}

\begin{table}
\setlength{\tabcolsep}{2 pt}
\centering
\renewcommand{\arraystretch}{1.1}
  \caption{Bugs found by different fuzzers on LAVA-M datasets}
  \label{tab:lava}  
  \begin{tabular}{lrrrrrrrr}
    \toprule
    \multirow{2}{*}{Programs} & \multirow{2}{*}{Listed} & \multicolumn{7}{c}{number of bugs } \\\cline{3-9}
    & &FUZZER  & SES & Vuzzer & Steelix & Angora & lafintel & NEUZZ \\
    \midrule
    base64 & 44 & 7 & 9 & 17 & 43 & 48 & 42 & 48\\
    md5sum & 57 & 2 & 0 & 1 & 28 & 57 & 49 & 60 \\
    uniq & 28 & 7 & 0 & 27 & 24 & 29 & 24 & 29 \\
    who & 2136 & 0 & 18 & 50 & 194 & 1541 & 0 & 211\\
  \bottomrule
\end{tabular}
\end{table}
The LAVA dataset is a metric to evaluate efficacy of fuzzers by providing a sets of real-world programs injected with a large number of realistic bugs ~\cite{lava}. LAVA-M is a subset of LAVA datasets, consisting of $4$ GNU coreutil programs base64, md5sum, uniq and who, respectively injected with 44, 57, 28, 2136 bugs. All bugs are guarded by a four-bytes magic number comparison. If the condition is satisfied, then the bug number will be printed out, meanwhile an out-of-bound memory read/write would occur and crash the tested program. 

Triggering a magic number condition is a hard task for a coverage-guided fuzzer because the fuzzer has to generate the exact combination of four contentious bytes out of $256^4$ possible cases. And \sys needs program inputs generated by a coverage-guided fuzzer to learn a surrogate neural program. If all the program inputs didn't trigger the magic number condition, then the corresponding labels for that magic condition would be all $0$ and neural program would learn nothing for this magic condition. To solve this program, we use AFL-lafintel to transform a magic byte comparison into four nested byte-comparisons. To trigger a byte-comparison is a easier task for a coverage-guided fuzzer than a magic-byte comparison since the searching space is reducing from $256^4$ to $256$. We run AFL-lafintel for an hour to generate program inputs as training data, then train a neural program whose gradient identify the possible critical bytes triggering the first byte-comparison of a magic-byte condition. After we successfully locate the critical byte by searching all possible critical bytes (we choose top $100$ critical bytes, each byte have $256$ possible values, total $25600$ tries), we perform a local exhaustive search to the adjacent byte of the critical bytes to break the second byte-comparison in $256$ tries, then another $256$ tries to break the third byte-comparison, then the last $256$ tries to break the fourth byte-comparison. Therefore, we only need 1 time gradient computation and $26368$ tries to trigger each bug. We also observed great results by AFL-lafintel itself when collecting training data. So we re-split 4 hours time budget to AFL-lafintel to collect training data and leave 1 hour to perform efficient searching guided by neural program.  

LAVA-M dataset has been evaluated by multiple state-of-the-art fuzzers with $5$ hours time budget, including a coverage-guided fuzzer (FUZZER), a symbolic execution tool (SES)~\cite{lava}, Vuzzer~\cite{vuzzer}, Steelix~\cite{steelix}, Angora~\cite{chen2018angora} and T-fuzz\dng{add t-fuzz reference}. We compare \sys with all these fuzzers and the result are summarized in table~\ref{tab:lava}. We also observed great results by AFL-lafintel when collecting training data, so we listed the 5 hours fuzzing result of AFL-lafintel on the table. \sys finds all the bugs in programs base64, md5sum and uniq, and second highest bug number in program who.  Note that LAVA-M authors left some bugs unlisted in all $4$ programs, so the total number of bugs found by \sys can be higher than the number of listed bugs. We explain the reason for \sys's promising results as follows. 

First, all the bugs in LAVA-M datasets, guarded by a four-byte magic number condition, can be triggered by four consecutive bytes in the program input. \sys uses AFL-lafintel to transform the four-byte magic number comparison into four nested byte-comparisons. AFL-lafintel can easily trigger the first byte-comparison easily by randomly fuzzing, but it cannot locate the critical byte which determines the first byte-comparison. Given the program inputs generated by AFL-lafintel, \sys can learn a neural program which help identify the possible critical bytes in the program inputs leading to first byte-comparisons. Then it just need another $256*3$ tries to perform a local exhaustive search to break the complex magic number comparisons, which greatly reduce the searching space. However, the transformation of magic number comparison by AFL-lafintel would cause a potential edge explosion issue for programs with a large number of compare instructions. The large number of edges emitted by AFL-lafintel would cause frequent edge conflict in the AFL edge map. This explains why AFL-lafintel cannot find any bugs in program who, and edge explosion also affects \sys performance on program who. 

Second, most of fuzzers (except) fails to find most of bugs in program md5sum because the improper seed provided by LAVA-M would cause the program to run slowly. We followed the latest suggestion on the authors of LAVA-M's blog, reduce the seed of md5sum into a single line, which greatly boost the fuzzing performance. 

Third, compared with Steelix and Vuzzer which leverage magic number hard-coded in the binary to construct a program inputs, \sys's locally exhaustive searching strategy do not rely on any hard-coded magic number, thus it can find all the bugs in program md5sum which requires some computations of input bytes to do the magic number checking. Compared with Angora, the best-performed LAVA-M fuzzer, \sys find $3$ more bugs unlisted bugs in program md5sum than angora because \sys do not need to solve the complex magic number condition at one time, as long as it can trigger the first byte-comparisons of a magic number condition, it can trigger the bug quickly. While Angora have to solve every complex magic number conditions and it's hard to hit all of them given fixed time budget. Angora finds $1541$ in program who, while \sys only find $211$ bugs because AFL-lafintel transformation generates too many additional edges which cause a sever edge conflict issue. We try to expand the edge map size to mitigate this issue, but find that AFL-lafintel cannot fully explore all the first byte-comparisons of all $2136$ magic number comparisons within limited time budget, which limit the accuracy of neural programs learnt from pro rams inputs generated by AFL-lafintel. 
                  
\input{RQ_tab}
\input{RQ_fig}

==> tables/experiment.tex <==
% \begin{table}[!t]
% \setlength{\tabcolsep}{3.5pt}
% \centering
% \scriptsize
% \renewcommand{\arraystretch}{1.1}
% 	\caption{\textbf{\small Experimental Setting}}
% 	\label{tab:experiment}  
%   \begin{tabular}{lll}
%     \toprule
%     & \textbf{Experiment}    & \textbf{Budget} \\\midrule
%   Evolutionary & 10 real-world programs & 24 hours fixed time\\
%   Fuzzers & LAVA-M datasets        & 5 hours fixed time \\
%   (RQ1 \& RQ2) & CGC datasets           & 6 hours fixed time \\
%     \midrule
%   Learning-based & \multirow{2}{*}{\sys vs. RNN (RQ3)} & a.Training time cost. \\
%   Fuzzers &                    & b. 1 million fixed mutations \\
%     & different variations of \sys (RQ4) & Fixed number of mutations\\
%   \bottomrule
% \end{tabular}
% % \tableshrink
% \end{table}

\begin{table}[!t]
\setlength{\tabcolsep}{3.5pt}
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1}
	\caption{\textbf{\small Experimental Setting}}
	\label{tab:experiment}  
  \begin{tabular}{lll}
    \toprule
    \textbf{Experiment}    & & \textbf{Budget} \\\midrule
    \multicolumn{3}{c}{Evolutionary Fuzzers (RQ1 \& RQ2)} \\\midrule
    & 10 real-world programs &   24 hours fixed time\\
    (RQ1 \& 2) & LAVA-M dataset        &   5 hours fixed time \\
    & CGC dataset           &    6 hours fixed time \\
    \bottomrule
    \multicolumn{3}{c}{Learning-based Fuzzers} \\\midrule
    \multirow{2}{*}{(RQ3)} & \multirow{2}{*}{\sys vs. RNN} &  a. Training time cost \\
                                  && b. 1 million fixed mutations \\
     (RQ4) & Different variations of \sys &  Fixed number of mutations\\
  \bottomrule
\end{tabular}
% \tableshrink
\end{table}



==> tables/fuzzer_desc.tex <==
\begin{table}[]
\setlength{\tabcolsep}{3pt}
\centering
\renewcommand{\arraystretch}{1.1}
  \caption{\textbf{\small Studied Fuzzers}}
  \label{tab:fuzzer_tech}  
\begin{tabular}{l|p{0.7\columnwidth}}
\toprule
Fuzzer & Technical Description \\
%\midrule
%\multicolumn{2}{c}{\textbf{Fuzzers with Source Code}}\\
\midrule
\afl~\cite{afl} & evolutionary searching \\
\aflfast~\cite{aflfast} & evolutionary + markov models searching\\
\vuzzer~\cite{vuzzer} & evolutionary + dynamic taint guided searching  \\
\kleefl~\cite{kleefl} & evolutionary searching + seeds generated by symbolic execution\\
%\midrule
\lafintel~\cite{lafintel} & evolutionary searching + compare instruction transformation\\
RNNfuzzer~\cite{rajpal2017not} & evolutionary searching + RNN-guided mutation filter\\
Angora~\cite{angora} & evolutionary + dynamic taint guided + black-box gradient descent guided searching + type inference + context sensitive edge coverage\\
steelix~\cite{steelix} & evolutionary searching + comparison progress feedback\\
T-fuzz~\cite{tfuzz} & evolutionary searching + program transformation\\
%\sys  & A NN-based fuzzer to generate mutated inputs with the guidance of neural program \\         
\bottomrule 
\end{tabular}
\end{table}

==> todo-list.tex <==
1. mention that \sys is flexible and can be combined with any existing fuzzers by train a NN model with their input corpus.  
